Joker: Conditional 3D Head Synthesis with Extreme Facial Expressions

We introduce Joker, a new method for the conditional synthesis of 3D human heads with extreme expressions. Given a single reference image of a person, we synthesize a volumetric human head with the reference identity and a new expression. We offer control over the expression via a 3D morphable model (3DMM) and textual inputs. This multi-modal conditioning signal is essential since 3DMMs alone fail to define subtle emotional changes and extreme expressions, including those involving the mouth cavity and tongue articulation. Our method is built upon a 2D diffusion-based prior that generalizes well to out-of-domain samples, such as sculptures, heavy makeup, and paintings while achieving high levels of expressiveness. To improve view consistency, we propose a new 3D distillation technique that converts predictions of our 2D prior into a neural radiance field (NeRF). Both the 2D prior and our distillation technique produce state-of-the-art results, which are confirmed by our extensive evaluations. Also, to the best of our knowledge, our method is the first to achieve view-consistent extreme tongue articulation.

==> sec/3_preliminaries.tex <==
\section{Preliminaries}

\paragraph{Latent Diffusion Models}
Diffusion models are a class of generative models that synthesize samples by autoregressive denoising of Gaussian noise $z_T~\mathcal{N}(0,1)$ through $T$ denoising steps.
%
Latent diffusion models~\cite{rombach2021highresolution} perform the denoising operation in the latent space of a pretrained variational autoencoder (VAE) using text conditionings as guidance.
%
At training time, images $x_0$ are projected to their latent space representation $z_0$ through the pretrained VAE encoder $\mathcal{E}$: $z_0=\mathcal{E}(x_0)$.
%
Random noise $\epsilon$ is applied to obtain a noisy latent vector $z_t$ that serves as input to the diffusion model $\epsilon_\theta$. The diffusion model is trained to estimate the added noise from the noisy observation: 
%
\begin{equation}
    L_\text{ldm} = \mathbb{E}_{z_0, c_\text{text}, t, \epsilon  \sim \mathcal{N}(0,1)} \left[\left|\left|\epsilon - \epsilon_\theta\left(z_t, c_\text{text}, t\right)\right|\right|_2^2\right].
\end{equation}
$\epsilon_\theta$ is parametrized as a UNet architecture with ResNet blocks, conditioned on the denoising time step and the text.
%



\paragraph{Basel Face Model}
The Basel Face Model (BFM) \cite{bfm09} is a 3D Morphable Model (3DMM) that represents the space of plausible 3D meshes of human faces with a PCA basis to model the identity and blendshapes to model expressions. 
%
A face is parametrized by $\alpha \in \mathbb{R}^{80}, \beta\in\mathbb{R}^{64}, \text{and} \gamma \in \mathbb{R}^{6}$ which denote parameters for identity, expression, and rigid transformation respectively.
%
The BFM maps these parameters to a mesh $\mathcal{M}\in\mathbb{R}^{36k\times3}$.
%
\begin{equation}
    \text{BFM}: \alpha, \beta, \gamma \mapsto \mathcal{M}.
\end{equation}


\paragraph{Neural Radiance Fields}
Neural Radience Fields (NeRF) \cite{mildenhall2020nerf} are a volumetric representation for 3D scenes through optical density and radiance fields parametrized by multi-layer perceptrons (MLP).
%
The MLP maps 3D location and view direction to a color value c and opacity $\theta$. For rendering images, rays are cast into the 3D volume, and optical density and color are queried along the rays. 
%
Volumetric integration yields the final pixel color prediction. During optimization, the reconstruction error between NeRF prediction and ground truth images is minimized. 




